GEOPHYS: The Geometry of Physical Plausibility

While humans can identify physically implausible events within milliseconds, machine learning approaches addressing the same problem are extremely slow and expensive. They either rely on external multimodal-LLM judges or require ad-hoc modifications to the training procedure. In this work, we argue that indicators of physical plausibility are implicitly captured by five geometric properties of the per-frame embeddings produced by frozen image encoders. In aggregate, we call them GEOPHYS. First, we show that these signals correlate with human EEG responses to two forms of object-permanence violations. Second, GEOPHYS robustly discriminates physically implausible videos from realistic ones, achieving state-of-the-art physics-violation detection: 98.3% on LikePhys and 93.3% on IntPhys2, whereas V-JEPA 2, GPT-4o, Gemini, and twelve modern video diffusion models perform near chance. Third, used as a best-of-N verifier for physical alignment during video generation, GEOPHYS lifts MAGI-1 24B from 50.01% to 64.50% on PhysicsIQ at 1.5x lower wall-clock and 4.65x lower memory than the V-JEPA 2 world-model verifier. Ultimately, GEOPHYS demonstrates that physical plausibility in videos can be assessed by leveraging the emergent geometric properties of temporal features extracted from image encoders.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Limitations parapgraph in Conclusion
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See Evaluation and Appendix
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes via bootstrap, see Evaluation setup
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See computation analysis in Evaluation
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> figures/pre_post_table.tex <==
\newcommand{\hmcellprepost}[1]{%
  \ifnum#1>75\cellcolor[RGB]{70,160,70}\textbf{#1}%
  \else\ifnum#1>40\cellcolor[RGB]{170,215,170}#1%
  \else\ifnum#1>0\cellcolor[RGB]{210,235,210}#1%
  \else\ifnum#1=0\cellcolor[RGB]{255,255,255}#1%
  \else\ifnum#1>-40\cellcolor[RGB]{240,180,175}#1%
  \else\cellcolor[RGB]{220,100,90}#1%
  \fi\fi\fi\fi\fi%
}
\begin{table}[h]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{ll cc}
\toprule
\textbf{Backbone} & \textbf{Signal} & \textbf{Create} & \textbf{Vanish} \\
\midrule
\multicolumn{4}{l}{\textit{CORnet-S}} \\
& Speed & \hmcellprepost{-40} & \hmcellprepost{100} \\
& Acceleration & \hmcellprepost{-44} & \hmcellprepost{85} \\
& Curvature & \hmcellprepost{0} & \hmcellprepost{-7} \\
& Angle Consistency & \hmcellprepost{0} & \hmcellprepost{7} \\
& Prediction Error & \hmcellprepost{-44} & \hmcellprepost{85} \\
\multicolumn{4}{l}{\textit{DINOv2}} \\
& Speed & \hmcellprepost{-1} & \hmcellprepost{1} \\
& Acceleration & \hmcellprepost{-2} & \hmcellprepost{2} \\
& Curvature & \hmcellprepost{-4} & \hmcellprepost{28} \\
& Angle Consistency & \hmcellprepost{4} & \hmcellprepost{-26} \\
& Prediction Error & \hmcellprepost{-2} & \hmcellprepost{2} \\
\multicolumn{4}{l}{\textit{DINOv3}} \\
& Speed & \hmcellprepost{42} & \hmcellprepost{-42} \\
& Acceleration & \hmcellprepost{100} & \hmcellprepost{-1} \\
& Curvature & \hmcellprepost{13} & \hmcellprepost{43} \\
& Angle Consistency & \hmcellprepost{-12} & \hmcellprepost{-43} \\
& Prediction Error & \hmcellprepost{100} & \hmcellprepost{-1} \\
\multicolumn{4}{l}{\textit{VOneNet}} \\
& Speed & \hmcellprepost{-2} & \hmcellprepost{5} \\
& Acceleration & \hmcellprepost{-4} & \hmcellprepost{9} \\
& Curvature & \hmcellprepost{-3} & \hmcellprepost{1} \\
& Angle Consistency & \hmcellprepost{2} & \hmcellprepost{-1} \\
& Prediction Error & \hmcellprepost{-4} & \hmcellprepost{9} \\
\bottomrule
\end{tabular}
\caption{Mean valid $-$ invalid signal post-occlusion (baseline-subtracted,
         scaled to $[-100, 100]$). Green = violation detected; red = wrong direction.}
\label{tab:prepost}
\end{table}

==> old.tex <==
%====================================================================
\section{Introduction (TODO)}
\label{sec:intro}
%====================================================================

Video generation models produce visually compelling outputs~\cite{wan2025,cogvideox2024,mochi2024} but routinely violate basic physics---objects pass through walls, gravity acts inconsistently, collisions produce implausible trajectories \citep{bear2021physion}. The dominant response has been to build bespoke machinery for the problem: physics-specific pretraining~\cite{yuan2025newtongen,chefer2025videojam}, physics-specific reward models trained on large world-modelling corpora~\cite{yuan2026wmreward}, or multimodal language models prompted to judge plausibility~\cite{yuan2026wmreward}. Each of these solutions assumes that the signal for physical plausibility must be \emph{added} to a vision system.

We show that a version of that signal is already present---not as physical knowledge, but as the temporal plausibility structure that pretrained vision models pick up from natural video.

\paragraph{A discovery, not just a framework.}
Our central finding is that the \emph{temporal plausibility} of a video--- i.e., how well a sequence of frames respects the natural-scene statistics that pretrained vision models are exposed to---is encoded, implicitly but measurably, in the geometry of feature-space trajectories. We do not claim these models reason about physics. Instead, two classical ideas from computational neuroscience predict such an effect without invoking physics at all.
The \emph{perceptual straightening hypothesis}~\cite{henaff2019straightening,henaff2021straightening} posits that natural video trajectories become geometrically straighter in biological visual cortex and in models that mimic it, making temporal prediction tractable in feature space where it is intractable in pixel space.
\emph{Predictive coding}~\cite{rao1999predictive,friston2010freeenergy} proposes that visual processing minimises the error of these predictions, propagating only the deviation between what was expected and what was seen.
Together, these ideas suggest a sharp empirical prediction: \emph{videos that match the natural dynamics encoded by a pretrained model should produce smooth, predictable feature-space trajectories, while videos that depart from those dynamics should break them}. Physical violations (objects passing through walls, gravity acting inconsistently, trajectories skipping in time) are a natural special case of such a departure, since natural videos rarely contain them. We test this prediction directly across four architecturally distinct backbones---self-supervised vision transformers (DINOv2, DINOv3), a recurrent convolutional model of the ventral visual stream (CORnet-S), and a biologically-constrained network with a fixed Gabor V1 front-end (VOneNet)---on benchmarks originally designed to test physics understanding. The prediction holds: the geometry of feature-space trajectories separates plausible from implausible videos, often by large margins and always without training.

Three aspects of this finding are non-obvious and make the paper's scientific contribution:

\textbf{(i) Physics emerges from objectives that are not about physics.} DINOv2 is trained to match masked views; DINOv3 adds register tokens; CORnet-S is trained for ImageNet classification with a recurrence prior; VOneNet is a ResNet with a fixed biologically-motivated front-end. None of these objectives involves physics, yet all four backbones produce feature geometries that discriminate physics violations above every published baseline.

\textbf{(ii) Neuro-inspired models are the strongest for localised violations.} On IntPhys2---which tests object permanence, solidity, continuity, and immutability---the \emph{V1-like} layers of the neuro-inspired models (VOneNet's Gabor block and CORnet-S's V1 module) achieve the highest single-backbone accuracy, outperforming both their own deeper layers (CORnet-S~IT) and the self-supervised ViTs. Biologically-constrained early visual features, which preserve fine spatial structure, turn out to be unusually well-matched to a task they were never designed for.

\textbf{(iii) The four backbones are complementary.} Each backbone catches violations the others miss. On LikePhys, VOneNet is strongest on fluid dynamics while DINOv3 uniquely captures river dynamics; on IntPhys2, different backbones dominate different conditions (permanence, immutability, solidity). This complementarity recovers 20+ points of accuracy when the four backbones are combined by a simple majority vote, suggesting that temporal-plausibility sensitivity is distributed across the vision-model landscape rather than concentrated in a single architecture.

\paragraph{From discovery to framework.}
Having established that this latent signal exists, we build \ours{}, a minimal framework to extract and deploy it. \ours{} computes two families of geometric signals on frozen backbone features---kinematic signals (speed variation, acceleration, angle consistency) for trajectory-level violations, and spatial-aware signals (cross-occlusion token matching, T$\times$T activity dissimilarity) for localised semantic violations---and uses them in three applications (Section~\ref{sec:experiments}): physics-violation detection on LikePhys and IntPhys2, temporal signal analysis with a comparison to human fMRI responses under matched violation-of-expectation stimuli~\cite{liu2024voe}, and best-of-$N$ selection for improving physical plausibility in generated video.

Our contributions are:
\begin{enumerate}
    \item The empirical finding that frozen pretrained vision backbones---including self-supervised ViTs and biologically-motivated models trained on unrelated objectives---encode temporal plausibility in the geometry of their feature-space trajectories, consistent with the perceptual straightening and predictive-coding hypotheses, with neuro-inspired V1-like layers emerging as the strongest single detectors for localised violations.
    \item \ours{}, a training-free framework that operationalises this finding through two families of geometric signals computed on frozen features, requiring no model access, no finetuning, and no labelled physics data.
    \item State-of-the-art physics-violation detection on both benchmarks tested---97.7\% on LikePhys and 93.3\% on IntPhys2 with the OR ensemble; 91.9\% / 77.5\% at majority vote. Every individual backbone exceeds all published baselines on both benchmarks.
    \item A per-frame temporal signal analysis that identifies \emph{when} valid and invalid videos diverge, enabling a direct comparison with EEG physical violation responses in humans viewing matched violation-of-expectation stimuli (ongoing work, Sec.~\ref{sec:temporal}).
    \item A best-of-$N$ video-selection strategy that improves PhysicsIQ by +15.6 points using kinematic acceleration alone, competitive with trained reward models that require much larger generators and proprietary components.
    \item A task-dependence finding: detection benefits from signal \emph{diversity} across backbones, while best-of-$N$ selection benefits from signal \emph{specificity} within a single backbone. Ensembling helps one application and hurts the other, suggesting that different aspects of the same latent plausibility signal serve different downstream uses.
\end{enumerate}







\subsection{Study 1: Temporal signal analysis}
\label{sec:neuro}

\begin{center}
\includegraphics[width=1\textwidth]{figures/neurofig_v2.png}
\end{center}
\captionof{figure}{
\textbf{Detecting object permanence violations in models and brains. }
(a) Example VOE stimuli for the Create scenario: in valid videos, one object enters and exits occlusion; in the invalid videos, one object enters but two exit. (b–c) valid and invalid Create signals from \ours{} CORnet-S IT (speed) (b) and EEG contralateral delay activity (from \cite{balaban2024electrophysiology}; c).  Both \ours{} and brain signals are elevated for the invalid condition after occlusion offset (vertical dashed line). (d–e) Mean valid - invalid \ours{} CORnet-S IT speed from pre- and post-occlusion windows of the Create (d) and Vanish (e) scenarios (rendered with ADEPT). In Vanish scenarios, the valid condition featured two objects. The EEG 'lag' period encompasses occlusion offset and the known neural resetting window following permanence violations \cite{balaban2024electrophysiology}.}
\label{fig:4_Neuro}

\paragraph{Setup.}

% TODO: 3-4 sentences explaining the alignment metric. Reviewers
% will flag the table without this. Tentative skeleton:
% (1) For each backbone × stimulus, we compute the per-frame signal
%     trace and align it to the EEG/MEG surprise window from each
%     study (Balaban: ___; Liu: ___; Kaiser: ___).
% (2) Alignment score = ___ (e.g., proportion of trials where signed
%     valid-vs-invalid difference matches EEG sign in the post-onset
%     window, or peak-to-peak temporal correlation, or...).
% (3) Score of 100 = perfect agreement, 50 = chance, 0 = anti-aligned.
% \fp{Ok, I get your point but in my mind this reads as: I found something in the models, then I justify it biologically, then I go back to implementing the models. Typically papers try to go from motivation to practical impact/consequences. Maybe because some LLM-as-a-judge evaluations haven't been done for physics violation, but I perceive physics violation WAY MORE practical (cause it's used e.g. for reward signal modelling whent raining models) than temporal signal analysis. So I'd rather go from 'this thing is biologically grounded, as it discriminates in the biological field, it also does so in the machine learning field, and there it has a practical impact in LLM-as-a-judge. And as a consequence there's an impact on generation ability}
% Detection establishes \emph{that} the geometric signal exists;
% straightening establishes \emph{why} it should. A more demanding test is whether the signal also tracks \emph{when} a violation occurs. The violation of expectation (VOE) paradigm from cognitive neuroscience has repeatedly demonstrated time-locked neural and behavioral responses to unexpected --- including physically impossible --- events in infants and adults~\cite{spelke1990core, baillargeon1985object}.
% Using several stimulus sets designed under this framework~\cite{}, we first validate that \ours{} detects VOE videos showing violations
% of object permanence, solidity, and material behavior, using the aggregated scores $u^{(b)}_{\phi}(\vect{V})$ defined in
% Sec.~\ref{sec:method_signals}. \fp{The part about VOE is completely incomprehensible without a background in the topic. I would suggest rewriting it by taking a baby-steps approach for the ML reader, and not the CogSci reader. In particular a solution to this problem is the following: To show \ours{} can detect unexpected, including physically impossible, videos, we rely on the well-established Violation of Expectation (VOE) approach from cognitive neuroscience. This proposes standardised experiments that have been repeatedly used to identify (time-locked??? what does this even mean???) neural and behavioural responses to such anomalous visual stimuli in infants and adults. We proceed as follows: (turn the sequence of things you do into bulletpoints, there's many steps here and it's hard to follow what thing you do serves what purpose in the global chain that constructs the experiment: until you reach the end it's not clear how the things concatenate to the point you want to support. E.g. Start with: To measure how consistently geophys signals are between valid and invalid videos after the moment of violation, we (the stuff that comes before). in general american-centric storytelling goes from very simple, clear and immediate (motivation, result)-tuple to steps made to get to the result. Motivation must be brief to justify the utility and impact of the result. You need to first raise the interest and motivate why they should bother reading all the details, and then once they understood why, you flood them with details and they can cognitively associate them to the purpose you clarified to them already} We then focus on two object permanence scenarios --- Create and Vanish
% --- in which valid videos show a consistent number of objects entering and exiting occlusion, while invalid videos show one more (Create) or one fewer (Vanish) object exiting than entered. For one instance of each scenario, we retain the per-frame quantities
% $(\theta_t, s_t, \vect{a}_t, \vect{\varepsilon}_t)$ defined in
% Sec.~\ref{sec:method_signals} and measure how well \ours{} temporal dynamics align with human EEG responses
% from~\cite{balaban2024electrophysiology} ($n=16$ subjects),
% specifically examining the contralateral delay activity (CDA) --- a biomarker of visual working memory that is modulated by physical expectation violations and the number of objects in a scene. Using additional VOE datasets and stimuli generated with
% ADEPT~\cite{smith2019modeling}, we further measure how consistently \ours{} signals diverge between valid and invalid videos after the moment of violation.
% Detection establishes \emph{that} the geometric signal exists;
% straightening establishes \emph{why} it should. A more demanding
% test is whether the signal also tracks \emph{when} a violation occurs. 
% \FP{This paragraph does not introduce what we are doing. I think we should clearly specify what is the task and what we're trying to do}To determine whether \ours{} can precisely track  \emph{when} a violation occurs, and carries meaningful (i.e., biologically-plausible) signal, we rely on the violation of expectation (VOE) paradigm from cognitive neuroscience. VOE approaches use standardised stimuli to reliably elicit infant surprise responses to physically impossible events~\cite{margoni2024violation, dunn2017investigating}.
% Recently, the VOE paradigm has been extended to adult EEG recordings, showing that object permanence violations trigger immediate and persistent shifts in brain activity~\cite{balaban2024electrophysiology}. We address whether \ours{} signals mirror these immediate and persistent shifts, and are sufficient for physical violation detection on paired VOE stimuli across two experiments: 

To determine whether \ours{} can precisely track \emph{when}
a violation occurs and carries meaningful (i.e., biologically
plausible) signal, we rely on the violation of expectation (VOE)
paradigm from cognitive neuroscience, which uses standardised stimuli
to reliably elicit surprise responses to physically impossible events
in infants ~\cite{margoni2024violation, dunn2017investigating}.
Recently, the VOE paradigm has been extended to adult EEG recordings,
showing that object permanence violations trigger immediate and
persistent shifts in brain activity~\cite{balaban2024electrophysiology}.
In a qualitative study, we seek to find similar signals in \ours{}.
In a quantitative study, we measure the reliability of such signals and overall detection performance.
We address both across two experiments:

\begin{enumerate}

\item \textbf{Biological alignment.} Using neural data and a subset
of publicly available stimuli from~\cite{balaban2024electrophysiology},
we qualitatively compare \ours{} per-frame signals
$(\theta_t, s_t, \vect{a}_t, \vect{\varepsilon}_t)$ to the
contralateral delay activity (CDA), an established EEG marker
of visual working memory known to (1) rapidly reconfigure
following expectation violation and (2) scale with the number of
objects in a scene~\cite{balaban2024electrophysiology,
ikkai2010contralateral, mccollough2007electrophysiological}.
EEG was recorded from $n = 16$ human subjects viewing two VOE
object permanence scenarios: Create, where one object entered an
occluder but two emerged, and Vanish, where two objects entered
but only one emerged, alongside matched valid controls.

\item \textbf{Signal reliability.} To test whether \ours{} signals reliably track changes in object number, we first generate additional videos with ADEPT, a VOE stimulus generator ~\cite{smith2019modeling}.
For each paired video, we compute the difference between valid and invalid per-frame signals pre-occlusion, when valid and invalid videos match, and post-occlusion, when objects appear (Create condition) or disappear (Vanish condition) from invalid videos. We finally validate \ours{}
aggregate detection performance $u^{(b)}_{\phi}(\vect{V})$ on these datasets.

% \item \textbf{Overall detection.} Finally, we validate \ours{}
% aggregate detection performance $u^{(b)}_{\phi}(\vect{V})$ on these and additional neuroscience VOE datasets, reporting results per backbone and for majority-vote and OR-gate ensembles.

\end{enumerate}
%────────────────────────────────────────────────────────────
\paragraph{Findings.}
% \fp{Where are the results? I can't find them. If you find them please put 'In Table/Figure X we show...'. From the rest of this section I really cannot understand what's going on, it's too incomplete this part.}
% \FP{At this point of reading I have no idea what the create scenario is, don't introduce terms that are not defined}
In the Create scenario (Fig.~\ref{fig:4_Neuro}a), both \ours{} CORnet-S IT speed signals (Fig.~\ref{fig:4_Neuro}b) and neural contralateral delay activity (Fig.~\ref{fig:4_Neuro}c) showed rapid and persistent increases in the invalid condition following the moment of violation. In the opposite Vanish scenario (Fig.~\ref{fig12: neuro_vanish_ts}a), both signals show a relative decrease in the invalid condition. Notably, unlike \ours{}, the CDA maintained elevated working memory representations during occlusion (${\sim}1.2$--$1.9$\,s), consistent with abstract object tracking beyond the visual input~\cite{balaban2024electrophysiology}. Quantitatively, \ours{} CORnet-S IT speed signals reliably tracked the number of objects in the scene (Fig.~\ref{fig:4_Neuro}d--e) in the Create scenario ($t(4) = 3.17$, $p = 0.03$). In the Vanish scenario, mean valid $-$ invalid signal diverged post-occlusion in the expected direction (valid $>$ invalid), but \ours{} was less sensitive to the total number of objects ($t(4) = -1.76$, $p = 0.15$), consistent with the weaker EEG Vanish effect reported in \cite{balaban2024electrophysiology}. Table~\ref{tab:prepost_transposed} reports the mean valid $-$ invalid difference across all backbones post-occlusion. CORnet-S IT speed, acceleration, and prediction error showed the only notable differences, with a relatively symmetric pattern across Create and Vanish. We additionally report per-backbone and ensemble \ours{} detection on the VOE stimuli (Table~\ref{tab:heatmap_neuro}).
% In the Create scenario (Fig.~\ref{fig:4_Neuro}a), both \ours{} CORnet-S IT speed signals (Fig.~\ref{fig:4_Neuro}b) and neural contralateral delay
% activity (Fig.~\ref{fig:4_Neuro}c) showed rapid and persistent
% increases in the invalid condition following the moment of violation, when
% two objects emerged from behind an occluder where only one had entered.
% In the opposite Vanish scenario (Fig.~\ref{fig12: neuro_vanish_ts}a), both
% signals show a relative decrease in the invalid condition following the
% disappearance of one of two objects originally occluded. Notably, unlike \ours{}, the CDA maintained elevated working memory 
% representations during occlusion (${\sim}1.2$--$1.9$\,s), consistent 
% with abstract object tracking beyond the visual input~\cite{balaban2024electrophysiology}. Quantitatively, \ours{} CORnet-S IT speed signals reliably tracked the
% number of objects in the scene (Fig.~\ref{fig:4_Neuro}d--e) in the Create scenario ( $t(4) = 3.17$, $p = 0.03$).  In the Vanish scenario, mean valid $-$ invalid signal diverged post-occlusion in
% the expected direction (valid $>$ invalid), but \ours{} was less sensitive to the total number of objects ($t(4) = -1.76$, $p = 0.15$) consistent with the weaker EEG Vanish effect reported in \cite{balaban2024electrophysiology}.
% Table~\ref{tab:prepost_transposed} reports the mean valid $-$ invalid difference
% across all backbones post-occlusion.
% CORnet-S IT speed, acceleration, and prediction error showed the only
% notable differences, with a relatively symmetric pattern across Create
% and Vanish. We additionally report per-backbone and ensemble \ours{} detection on the VOE stimuli (Table~\ref{tab:heatmap_neuro}).

% We additionally evaluated per-backbone and ensemble \ours{} detection on a broader set of
% VOE stimuli (Table~\ref{tab:heatmap_neuro}).
% Individual backbones achieved chance to moderate levels of performance: DINOv2 L12
% $66.8\%$ (angle consistency), DINOv3 L18 $50.0\%$ (angle consistency),
% CORnet-S IT $50.0\%$ (speed), and VOneNet V1 $68.8\%$ (acceleration),
% though we note the limited sample sizes ($n = 2, 3, 3$, and $3$ pairs,
% respectively).
% Majority vote was marginally above chance at $54.3\%$, while OR-gate
% detection was consistently $100\%$ across all datasets.

% %ts
\begin{takeaway}

\end{takeaway}
